VideoGUI: A Benchmark for GUI Automation from Instructional Videos

Graphical User Interface (GUI) automation holds significant promise for enhancing human productivity by assisting with computer tasks. Existing task formulations primarily focus on simple tasks that can be specified by a single, language-only instruction, such as "Insert a new slide." In this work, we introduce VideoGUI, a novel multi-modal benchmark designed to evaluate GUI assistants on visual-centric GUI tasks. Sourced from high-quality web instructional videos, our benchmark focuses on tasks involving professional and novel software (e.g., Adobe Photoshop or Stable Diffusion WebUI) and complex activities (e.g., video editing). VideoGUI evaluates GUI assistants through a hierarchical process, allowing for identification of the specific levels at which they may fail: (i) high-level planning: reconstruct procedural subtasks from visual conditions without language descriptions; (ii) middle-level planning: generate sequences of precise action narrations based on visual state (i.e., screenshot) and goals; (iii) atomic action execution: perform specific actions such as accurately clicking designated elements. For each level, we design evaluation metrics across individual dimensions to provide clear signals, such as individual performance in clicking, dragging, typing, and scrolling for atomic action execution. Our evaluation on VideoGUI reveals that even the SoTA large multimodal model GPT4o performs poorly on visual-centric GUI tasks, especially for high-level planning.

==> sections/checklist.tex <==
\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{All the claims made in the abstract and introduction are supported by the benchmark dataset, a new metric, and empirical evaluation.}
  \item Did you describe the limitations of your work?
    \answerYes{Given the expensive manual collection cost, \our~is limited by a smaller scale. Additionally, we provide final files but do not yet offer automatic success rate evaluation scripts, which require human validation.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo We do not see significant negative societal impacts from \our.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have reviewed the Code of Ethics.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{The paper does not include theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We will provide code, data samples and instructions in supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Training details are described in Appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We did not include error bars because experiments based on closed-source LLMs (\ie~API) are costly. Instead, we controlled parameters such as setting the temperature in LLM to 0 and provided all parameter settings and prompt template details.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Our work primarily focuses on data curation and evaluation. We conduct experiments on a machine with 4$\times$RTX6000 GPUs. The evaluation of \our~for all models costs approximately 150 USD.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We properly cited all code, data, and models used in this paper.}
  \item Did you mention the license of the assets?
    \answerYes{We provide MIT License software to be used with our data.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We provide data samples of our dataset in supplementary material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Our instructional videos are primarily sourced from YouTube with the consent of the video owners. We do not own the videos; instead, we provide the URL to refer to the original video link.}
    % But we discuss the similarity between our curated data and the recently released WebVid10M in supplementary material.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{The publicly available datasets from which our data is constructed do not have any PII instances and are devoid of toxic content.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{
    % We didn't conduct research with human subjects.
    Yes, since we focus on GUI software applications, we provide instructions to participants during data collection to ensure they understand the process and details. 
    }
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We didn't conduct research with human subjects.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/trainingdata.tex <==
\section{Instruction Data Generation} % Imitation Prompting
\begin{figure}[!b]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/training_pipeline.pdf}
	\caption{
 Illustration of the \ourdata instruction data generation pipeline.
}
\label{fig:demo}
\end{figure}

In this section, we demonstrate how can we harvest instruction-tuning corpus from scalable web instructional videos.
However, it is nontrivial to obtain these data, as the videos original provide noisy metadata and subtitles. While these visual information such as cursor action (click what) are not directly available. Thus, we propose a data curation pipeline to create high-quality instruction tuning corpus.
To meet the evaluation hierarchy, we also propose a paired data generation strategy to fill the gap.

\textbf{High-level:} 
One important channel to metadata and video subtitles. 
We can harvest the general information such as lesson topic or visual preview descriptions.
In this stage, we feed the metadata (video titles, description) as well as sentence-level subtitles into GPT4, and receive a series of high-level annotations.

\textbf{Middle-level:}
To get better alignment, we use WhisperX~\cite{} to obtain word-wise alignments. 
Besides, we found that the language models easily make mistake when proceed the fined-grained narrations. Thus, we design a Streaming strategy to handle this part.

\textbf{Atomic-level:}
In order to extract the cursor location from screenshots sequence in videos. We manual collect and label nearly 5K cursor annotations and then train a YOLO-v8 to learn such cursor detection ability.
However, as the video is not like simulate environment, we cannot obtain the button information (such as name and location) directly, we use the following OCR and Icon Template matching strategy. Based on the mouse location, we can navigate a region and then we obtain the spatial locations.
For OCR, we use the Microsoft OCR API to extract them, and for icon matching, we manually collect a icon databases, then we employ the pyramid matching to obtain.
Besides, as we need to associate the language narration with the element spatial information, thus, we assign a another language models.
